Revisiting Conventional Task Schedulers to Exploit Asymmetry in ARM big.LITTLE Architectures for Dense Linear Algebra

Dealing with asymmetry in the architecture opens a plethora of questions from the perspective of scheduling task-parallel applications, and there exist early attempts to address this problem via ad-hoc strategies embedded into a runtime framework. In this paper we take a different path, which consists in addressing the complexity of the problem at the library level, via a few asymmetry-aware fundamental kernels, hiding the architecture heterogeneity from the task scheduler. For the specific domain of dense linear algebra, we show that this is not only possible but delivers much higher performance than a naive approach based on an asymmetry-oblivious scheduler. Furthermore, this solution also outperforms an ad-hoc asymmetry-aware scheduler furnished with sophisticated scheduling techniques.

==> blis_gemm.tex <==
\begin{figure*}[t]
\centering
%\begin{tabular}{c}
%\begin{minipage}[c]{0.9\textwidth}
%\includegraphics[width=0.9\textwidth]{Figures/gotoblas_gemm.pdf}
%\end{minipage}\\
%\\
\begin{minipage}[c]{0.9\textwidth}
\scriptsize
\begin{tabular}{llll}
Loop 1 &{\bf for} $j_c$ = $0,\ldots,n-1$ {\bf in steps of} $n_c$, $\Jc = j_c:j_c+n_c-1$\\
Loop 2 & \hspace{3ex}  {\bf for} $p_c$ = $0,\ldots,k-1$ {\bf in steps of} $k_c$, $\Pc = p_c:p_c+k_c-1$\\
&\hspace{6ex}           \textcolor{darkblue}{$B(\Pc,\Jc)$} $\rightarrow \textcolor{darkblue}{B_c}$ & ~~~// Pack into $B_c$\\
Loop 3 & \hspace{6ex}           {\bf for} $i_c$ = $0,\ldots,m-1$ {\bf in steps of} $m_c$, $\Ic = i_c:i_c+m_c-1$\\
&\hspace{9ex}                     \textcolor{darkred}{$A(\Ic,\Pc)$} $\rightarrow \textcolor{darkred}{A_c}$ & ~~~// Pack into $A_c$ \\
%\cline{2-4} 
       &\hspace{9ex} \textcolor{darkgreen}{$C(\Ic,\Jc)$} := \textcolor{darkgreen}{$C(\Ic,\Jc)$} + 
                     \textcolor{darkred}{$A_c$} $\cdot$ \textcolor{darkblue}{$B_c$} & ~~~// Macro-kernel\\
%%%% Loop 4&\hspace{9ex} {\bf for} $j_r$ = $0,\ldots,n_c-1$ {\bf in steps of} $n_r$  & & // Macro-kernel\\
%%%% Loop 5&\hspace{12ex}   {\bf for} $i_r$ = $0,\ldots,m_c-1$ {\bf in steps of} $m_r$\\
%%%% \cline{2-3}
%Loop 6&\hspace{15ex}    {\bf for} $p_r$ = $0,\ldots,k_c-1$ {\bf in steps of} $1$ & // Micro-kernel \\
%%%% &\hspace{15ex}             \textcolor{darkgreen}{$C_c(i_r:i_r+m_r-1,j_r:j_r+n_r-1)$} & // Micro-kernel \\
%&\hspace{19ex} $:=$ ~\textcolor{darkgreen}{$C_c(i_r:i_r+m_r-1,j_r:j_r+n_r-1)$}\\
%%%% &\hspace{19ex} ~$\mathrel{+}=$     ~\textcolor{darkred}{$A_c(i_r:i_r+m_r-1,0:k_c-1)$} \\
%%%% &\hspace{19ex} ~~~$\cdot$\!~~~~\textcolor{darkblue}{$B_c(0:k_c-1,j_r:j_r+n_r-1)$} \\
%&\hspace{15ex} {\bf endfor}\\
%%%% \cline{2-3}
%&\hspace{12ex} {\bf endfor}\\
%\cline{2-4} 
&\hspace{6ex} {\bf endfor}\\
&\hspace{3ex} {\bf endfor}\\ 
&{\bf endfor}\\ 
\end{tabular}
\end{minipage}
%\end{tabular}
\caption{High performance implementation of \gemm in BLIS. In the code, %$C_c \equiv C(i_c:i_c+m_c-1,j_c:j_c+n_c-1)$
%is just a notation artifact, introduced to ease the presentation of the algorithm, while 
$A_c,B_c$ correspond to actual buffers that are involved in copies.}
\label{fig:gotoblas_gemm}
\end{figure*}

